RecShard: Statistical Feature-Based Memory Optimization for Industry-Scale Neural Recommendation

We propose RecShard, a fine-grained embedding table (EMB) partitioning and placement technique for deep learning recommendation models (DLRMs). RecShard is designed based on two key observations. First, not all EMBs are equal, nor all rows within an EMB are equal in terms of access patterns. EMBs exhibit distinct memory characteristics, providing performance optimization opportunities for intelligent EMB partitioning and placement across a tiered memory hierarchy. Second, in modern DLRMs, EMBs function as hash tables. As a result, EMBs display interesting phenomena, such as the birthday paradox, leaving EMBs severely under-utilized. RecShard determines an optimal EMB sharding strategy for a set of EMBs based on training data distributions and model characteristics, along with the bandwidth characteristics of the underlying tiered memory hierarchy. In doing so, RecShard achieves over 6 times higher EMB training throughput on average for capacity constrained DLRMs. The throughput increase comes from improved EMB load balance by over 12 times and from the reduced access to the slower memory by over 87 times.

==> 00-abstract.tex <==
\begin{abstract}

We propose RecShard, a fine-grained embedding table (EMB) partitioning and placement technique for deep learning recommendation models (DLRMs). RecShard is designed based on two key observations. First, not all EMBs are equal, nor all rows within an EMB are equal in terms of access patterns. EMBs exhibit distinct memory characteristics, providing performance optimization opportunities for intelligent EMB partitioning and placement  across a tiered memory hierarchy. Second, in modern DLRMs, EMBs function as hash tables. As a result, EMBs display interesting phenomena, such as the birthday paradox, leaving EMBs severely under-utilized. RecShard determines an optimal EMB sharding strategy for a set of EMBs based on training data distributions and model characteristics, along with the bandwidth characteristics of the underlying tiered memory hierarchy. In doing so, RecShard achieves over 6 times higher EMB training throughput on average for capacity constrained DLRMs. The throughput increase comes from improved EMB load balance by over 12 times and from the reduced access to the slower memory by over 87 times.

\end{abstract}

==> 05-casestudy.tex <==
\section{Case Study}
\label{sec:casestudy}


To measure the performance benefit of using RecShard we benchmark against various sharding schemes currently being used in production training systems. These production sharding schemes are generally defined by two components, a placement algorithm and a cost function [Mudigere-arxiv21].

The partition algorithms usable are two polynomial time heuristics, one being a greedy heuristic and the other being the largest differencing method (LDM). The greedy heuristic works as follows: first it calculates the cost per table using the chosen cost function, and then sorts the tables in descending cost order. It then allocates the largest cost tables first, placing one table per GPU. After this iteration completes it then continues down the list of descending cost tables, placing each table on the current GPU with smallest sum of costs. Once GPU memory has been filled the algorithm continues, allocating the remaining tables on UVM on a per-GPU basis. The LDM heuristic begins similarly, with tables sorted in descending cost order, but at each step takes the two largest cost values and replaces them in the list with their difference, acting as the placement of the two largest values in different partitions. It recursively continues this until the list is processed. When the heuristic completes it will yield a partition, which while not optimal, is generally better than the greedy heuristic. 

In order to perform their placements, the partitioning heuristics used in production require a cost function to evaluate and compare different embedding tables. Three cost functions we use in our evaluations are: 1) Size based, which uses the hash size of the table as its cost; 2) Lookup based, which uses the tables average pooling factor multiplied by its dimension as the cost; and 3) Hashed Lookup, which is the lookup based cost multiplied by the $log_{10}$ of the hash size to try and capture potential caching effects of smaller tables.

We evaluate the performance of RecShard against these 6 combinations of competing sharding schemes on 3 different production-scale models shown in Table \ref{table:model_desc}.


